Disentangling Generative Factors in Natural Language with Discrete Variational Autoencoders

The ability of learning disentangled representations represents a major step for interpretable NLP systems as it allows latent linguistic features to be controlled. Most approaches to disentanglement rely on continuous variables, both for images and text. We argue that despite being suitable for image datasets, continuous variables may not be ideal to model features of textual data, due to the fact that most generative factors in text are discrete. We propose a Variational Autoencoder based method which models language features as discrete variables and encourages independence between variables for learning disentangled representations. The proposed model outperforms continuous and discrete baselines on several qualitative and quantitative benchmarks for disentanglement as well as on a text style transfer downstream application.

==> tables/sentence_metric.tex <==
% proposed way to evaluate disentanglement in sentences
\begin{table} \small
\begin{tabular}{|l|l|p{2cm}|}
               \hline
               Score & Sentence Pair & Change \\ \hline
               \multirow{2}{*}{1}  & is he not suspending the user & S \\
               & is he suspending the user &  \\ \hline
               \multirow{2}{*}{0.8} & is he not suspending the user & S,G \\
               & is she suspending the user & \\ \hline
               \multirow{2}{*}{0.2} & is he not suspending the user & S,G,T,VO \\
               & was she moving the user & \\ \hline
               \multirow{2}{*}{0.0} & is he not suspending the user & S,G,T,VO,QA \\
               & she was moving the user & \\ \hline
\end{tabular}
\caption{Degrees of disentanglement} \label{tab:eval_dis1}
\end{table}


